On the Robust Approximation of ASR Metrics

Recent advances in speech foundation models are largely driven by scaling both model size and data, enabling them to perform a wide range of tasks, including speech recognition. Traditionally, ASR models are evaluated using metrics like Word Error Rate (WER) and Character Error Rate (CER), which depend on ground truth labels. As a result of limited labeled data from diverse domains and testing conditions, the true generalization capabilities of these models beyond standard benchmarks remain unclear. Moreover, labeling data is both costly and time-consuming. To address this, we propose a novel label-free approach for approximating ASR performance metrics, eliminating the need for ground truth labels. Our method utilizes multimodal embeddings in a unified space for speech and transcription representations, combined with a high-quality proxy model to compute proxy metrics. These features are used to train a regression model to predict key ASR metrics like Word Error Rate (WER) and Character Error Rate (CER). We experiment with over 40 models across 14 datasets representing both standard and in-the-wild testing conditions. Our results show that we approximate the metrics within a single-digit absolute difference across all experimental configurations, outperforming the most recent baseline by more than 50\%.

==> tables/qualitative-examples.tex <==
% Please add the following required packages to your document preamble:
% \usepackage[normalem]{ulem}
% \useunder{\uline}{\ul}{}
\begin{table*}[ht!]
\renewcommand{\arraystretch}{1.3} % Adjust row height for better readability
\setlength{\tabcolsep}{4pt} % Adjust column spacing
\footnotesize % Reduce font size

\begin{tabular}{p{5cm}p{5cm}p{1cm}p{1cm}p{1cm}p{1cm}p{1cm}}
\toprule
Ref                                                                                                                                                                                                                                                                                          & Hypothesis                                                                                                                                                                                                                                                                                           & WER      & aWER  & CER    & aCER  & Sim \\
\midrule
the hrv is not even on                                                                                                                                                                                                                                                                             & H R V IS NOT EVEN ON                                                                                                                                                                                                                                                                                 & 50.00    & 3.26  & 18.18  & 2.61  & 0.71       \\
% because my understanding is that it's because osha is sort of selffunding and they need to generate the revenue to support all these additional inspectors and things that they have decided will be their approach to safety as opposed to the programs like the vpp program and things like that & Because my understanding is that it's because OSHA is sort of self funding and they need to generate the revenue to support all these additional inspectors and things that they have decided will be their approach to safety as opposed to the programs like the VPP program and things like that. & 3.92     & 3.45  & 0.34   & 2.92  & 0.93       \\
CONSEIL WAS MY MANSERVANT                                                                                                                                                                                                                                                                          & conseil was my man's servant                                                                                                                                                                                                                                                                         & 75.00    & 7.39  & 12.00  & 5.54  & 0.88       \\
yeah so book an call support book an appointment to see and i will recommend that meet her face to face                                                                                                                                                                                            & yeah so book an appointment call support book an appointment to see and i would recommend that you do the face to face                                                                                                                                                                               & 23.81    & 19.78 & 22.33  & 11.21 & 0.87       \\
so she has money and then it turns out she's actually uber talented                                                                                                                                                                                                                                & has money she has money yeah and then it turns out she's actually talented                                                                                                                                                                                                                           & 28.57    & 28.63 & 25.37  & 19.12 & 0.56       \\
which is why the november 15th letter was sent asking to open the discussion about the two thousand and eighteen market season                                                                                                                                                                     & which is why the November 15th letter was sent asking to open the discussion about the 2018 market                                                                                                                                                                                                   & 22.73    & 23.45 & 25.40  & 39.91 & 0.91       \\
% Just looking into the fourth quarter firstly, I mean you've reiterated, clearly the guidance, the 10\% grade, you previously specified an H2 grade to get there, I think it would be 11 to 13\% and obviously we can sort of do the calculation around Q4.                                         & Just looking into the fourth quarter firstly, I mean you've reiterated clearly the guidance for the year ten percent growth. I mean, previously specified an H two growth to get there, I think it was eleven percent to thirteen percent and obviously you can sort of do the calculation around Q  & 36.96    & 17.06 & 30.00  & 10.69 & 0.82       \\
We'll continue to look at that and adjust targets as appropriate, but I'm not sure anything changes in terms of the big picture plan for South America. Yes, I mean I would say we are constantly benchmarking each of our countries                                                               & I would say we are constantly benchmarking each of our countries.                                                                                                                                                                                                                                    & 74.42    & 76.63 & 71.56  & 71.40 & 0.37       \\
% also have attached somewhat less less time in answering that question you have said that there is a progress on getting clarity on the guidelines there is an effort on your side and i'm sure that this is the case                                                                               & SO HAVE ATTACHED SOMEWHAT LESS LESS TIME IN ANSWERING THAT QUESTION YOU HAVE SETTLED THAT THERE IS A PROGRESS ON GETTING CLARITY ON THE GUIDE LINES THERE IS AN EFFORT ON YOUR SIDE AND I AM SURE THAT THIS IS THE CASE                                                                              & 12.20    & 26.75 & 4.25   & 14.37 & 0.72       \\
and you give him his carriage with his spats on and his cutaway uh coat you know and his top hat                                                                                                                                                                                                   & H GET IN HIS CARRIAGE WITH HIS SPATS ON AND HIS CUT AWAY COAT YOU KNOW AND HIS TOP HAT AND HIS CHAUFFEUR WOULD TAKE HIM OUT TO WITH THE HORSES NO LESS BEAUTIFULLY                                                                                                                                   & 95.24    & 19.78 & 95.83  & 10.09 & 0.71       \\
okay                                                                                                                                                                                                                                                                                               & I know it's called the "Gateway".                                                                                                                                                                                                                                                                    & 700.00   & 28.94 & 675.00 & 32.85 & 0.33       \\
foreign language.                                                                                                                                                                                                                                                                                  & tangzai sabungi tangzangan and kpanen simbolar to birlivian ain ojong meat aar reanded to it ingaru tampungid debi sampos and tethujun comes west mida                                                                                                                                               & 1,200.00 & 80.39 & 862.50 & 32.26 & 0.22       \\
stronger. our peoples and our economies                                                                                                                                                                                                                                                            & our peoples and our economies are tied                                                                                                                                                                                                                                                               & 50.00    & 14.44 & 47.37  & 8.17  & 0.87       \\
five dollar slaw onion cure                                                                                                                                                                                                                                                                        & \$5.00 Slaw Onion Care                                                                                                                                                                                                                                                                               & 60.00    & 44.22 & 40.74  & 27.24 & 0.74       \\
% foreign language.                                                                                                                                                                                                                                                                                  & thangtai thangtay thangangithanganang cepani simul chum buri lane lane jodong meet arranged to evoke chingaroo tompungi dee thump thump thump thang dee                                                                                                                                              & 1,100.00 & 86.33 & 868.75 & 55.95 & 0.17       \\
ignore\_time\_segment\_in\_scoring                                                                                                                                                                                                                                                                 & Look to Miguel. Farmers like Miguel.                                                                                                                                                                                                                                                                 & 120.00   & 6.84  & 86.67  & 4.02  & 0.92       \\
boy bout seventeen with a red cap no sir indeed i've not  \\   \bottomrule           
\end{tabular}
\caption{
Provide qualitative examples to showcase the effectiveness of our method. 
}
\end{table*}
